Quantifying Arbitrage in Automated Market Makers: An Empirical Study of Ethereum ZK Rollups

Arbitrage can arise from the simultaneous purchase and sale of the same asset in different markets in order to profit from a difference in its price. This work systematically reviews arbitrage opportunities between Automated Market Makers (AMMs) on Ethereum ZK rollups, and Centralised Exchanges (CEXs). First, we propose a theoretical framework to measure such arbitrage opportunities and derive a formula for the related Maximal Arbitrage Value (MAV) that accounts for both price divergences and liquidity available in the trading venues. Then, we empirically measure the historical MAV available between SyncSwap, an AMM on zkSync Era, and Binance, and investigate how quickly misalignments in price are corrected against explicit and implicit market costs. Overall, the cumulative MAV from July to September 2023 on the USDC-ETH SyncSwap pool amounts to $104.96k (0.24% of trading volume).

==> TODOs.tex <==

D: Pricing from Binance per 1 minute, 1H, 1D


form 1st July
abs price diff

time to realibment - decay time - when the price difference drops below threshold
- take max MAV in the perdios of disalighment


take distrinbutuon of price diff and take sigma

price diff in perctage

What is to-do:
a) add fees - SYncSwap USDC-ETH outstanding
a2) split fees into L1 and L2
b) add block slippage
c) add lp fees (8bps)
- maybe LP fees should be in the formula?
d) check with prices per second -

-> export of the currrent file (done)
-> export of the current file with fees, block splippage, ...

Questions to Debbie:
1) How to set the threshold for these 4 pools?
2) Does it make sense to check prices per second?

bl

AMMs
- data for centralized exchanges -> Binance
- DEX -> Uniswap v2
- on Ethereum it is 12 seconds - compare time dealy
- the largest 400 pools from Uniswap v2

--> threshold as \% of CEX price - DONE
--> distribution of ( price diff / CEX price ) - DONE
--> gas fee is in ETH -> to token0 (USDC, ETH) - DONE

TO DOs:
--.=> block slippage conitnue
--> let's make all fees like in Uniswap table absolute
--> threshold as boxplot max value (interqunatil range)

--> start writing the narrative (sth about Binnace, then about MAV and max MAV and decay
-> stats about decay and stats about MAX and max MAV

-> block slippage as change in reserves? how to make it a price impact?

Comments:
- #volume can be positive or negative, -> then implied slippage (the imbalance) -> descirbe more in the discussion part of the paper
- #also total sum withing a block
- disucssion - timing risk - when price changes too quickly


fees_avq_1m_0
fees_avg_upto_max_MAV_0

block_slippage_avg_1m_0
block_slippage_avg_upto_max_MAV_0

volume_total_upto_max_MAV_0
volume_avg_upto_max_MAV_0




diagram with MAX mav 

This framework is good for all later, not only zk but alos optymistic


New issues:
a) Threshold to high for ETH-BTC on zkSwap

b) calucaltions for usdc-eth for zkSwap


Other
- L1_fees vs L2_fees
- block slippage in bps (and other)
- price impact (in in bps)


market still inefficeint - some mav that are bigt and could be addressed fster
fees and size determine decay time, and 

Uniswap v3
zkSync - data 
Arbitrum is a must


There is no MEV auctions - 
underlying differnece with mainnet  -like block 2s (vs 12s) gaas ffee
How 


0) paper writing
1) Amount of swaps
2) Cite in Introduction
3) uniswap v3 trick
4) Pools with traded volume
5) Table with cost breakdown
6) Calculcations per second


-> table with fees (summary) -> how to desing
-> add that arbitrage is present on Uniswap v2 in methodology (Maveric is the largest DEX and zkSwap and 
-> add statistics 

FInish section 3 and 4
-> add LP fee vs MAV in bpd


0) change price diff, as AMM the same but at Binance it changes
1) DeFI Llama citation


NExt steps:
1) Maverlick (Uniswap v3) 

2) Block - 2s xkSYN
ETHEREUM - 12s
Arbitrum - 2s 


Dimention one:
Most active venue
2s-level (not minite with Biance)

Dimention two:
MAV oppprunes identifies vs Actual Exp;oite

L1<>L2 fees
- describe more, more on fidelity -> better characterize L2 ecosystem

more data
single swap analysis
1s data, L1<>L2

proof-of-storage
mint burn

Polaris

EIP upgrate - https://eips.ethereum.org/EIPS/eip-4844


1) Quantifying Arbitrage between Automated Market Makers on Ethereum zk-roll-ups and Centralised Exchanges
2) Price Disparities and Arbitrage between Automated Market Makers on Ethereum zk-roll-ups and Centralised Exchanges
3) Quantifying Arbitrage in Automated Market Makers. An Empirical study on Ethereum zk-roll-ups
4) Maximal Arbitrage Value in Automated Market Makers. An Empirical study on Ethereum zk-roll-ups
5) Maximal Arbitrageable Value in Automated Market Makers. An Empirical study on Ethereum zk-roll-ups


==> sections/OLD/04EmpiricalAnalysis.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Results}
%    \label{sec:analysis}


%Key questions:
%Historical gas costs?\\
%Historical data for Curve v1, v2 and Uniswap v2, v3\\
%-> List of swaps and their costs -> What is the average swap size? - do we really need this? Would spot price be enough?\\
%-> LP data about the pool compositions and sizes - reservers token 0, token 1 and LP-token (token supply)\\

%Plot with two dimensions - gas and defi costs
%-> Show where each chain stands

%Historical split of costs
%- average gas costs and defi costs 




==> sections/OLD/05Extensions.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Extensions}
    \label{sec:extensions}


\subsection{Further types of AMMs}



